Network-Aware Scheduling for Remote Gate Execution in Quantum Data Centers

Modular quantum computing provides a scalable approach to overcome the limitations of monolithic quantum architectures by interconnecting multiple Quantum Processing Units (QPUs) through a quantum network. In this work, we explore and evaluate two entanglement scheduling strategies-static and dynamic-and analyze their performance in terms of circuit execution delay and network resource utilization under realistic assumptions and practical limitations such as probabilistic entanglement generation, limited communication qubits, photonic switch reconfiguration delays, and topology-induced contention. We show that dynamic scheduling consistently outperforms static scheduling in scenarios with high entanglement parallelism, especially when network resources are scarce. Furthermore, we investigate the impact of communication qubit coherence time, modeled as a cutoff for holding EPR pairs, and demonstrate that aggressive lookahead strategies can degrade performance when coherence times are short, due to premature entanglement discarding and wasted resources. We also identify congestion-free BSM provisioning by profiling peak BSM usage per switch. Our results provide actionable insights for scheduler design and resource provisioning in realistic quantum data centers, bringing system-level considerations closer to practical quantum computing deployment.

==> problem.tex <==
\section{Motivation example and System model}

The gate-packing will happen at the neginign of the sub-circuit partitioning stage when we prepare the graph for the graph paritining algortithm or after we apply the graph partition and we modify the cost fo the graph partitioning algorithm even before comparing it with stikking with the previous partition or considerting the current partition plus the cost of moving the qubits. The reson is the cost of moving the states can not get benefit from gate packing. It is gate teleportation that can get benefit from gate packing. And gate teleportation is when we perform graph partitioning. 

\subsection{Problem}
We show an example that shows how the topology of the datacenter, the structure of the circuit, available resources on machines, and bandwidth  affects the entanglement generation and program latency.

We can assign flows with high rate to one pair of nodes and the other one will have zero. But how much delay this has on the memory decoherene needs to be evaluated. 

%In a quantum data center, we use multiple modules, called quantum processing units (QPUs) each holding a few qubits, and then execute an algorithm by doing single or multi-qubit gates on qubits possibly on different modules \cite{monroe2014large,jnane2022multicore}. Each two-qubit gate on two different QPUs consists of several tasks: (i) entanglement generation and distribution, (ii) local operations, and (iii) classical communications. The current challenge is to scale the system to very large sizes.


%Figure \ref{fig:FT_remote_gate} shows a topology of a QDC where at the lowest layer we have QPUs. At the upper layer, we have quantum storage servers where we have long-time storage servers. The entanglement between QPUs or storage servers can be generated via photonic switches. 





%In QDC, fast entanglement generation is required for executing a quantum algorithm with high fidelity. At the same time, not all pairs of QPUS would need entanglement at the same time due to the structure of the circuit of the algorithm. 

% The basis of quantum error correction (QEC) is storing and manipulating quantum information using logical qubits \cite{shor1995scheme}.  


% \begin{figure}
% \centering
%     \includegraphics[width=10cm]{img/FT_remote_gate.pdf}
%     \vspace{-0.06in}
%   \caption{Entanglement generation between two surface patches to perform a remote two-qubit gate. Entanglement purification may be required to improve the fidelity of the generated entanglements to reduce the logical error rate.\label{fig:FT_remote_gate}}
% \end{figure}


\myparab{Our proposal:} There are a few research questions that are worth exploring regarding using lattice surgery for distributed fault-tolerant quantum computing. \cite{ramette2023fault} explores the effect of noise in the generated entanglement for connecting multiple surface patches on the logical error rate but it does not consider the time that it takes to generate entanglement for connecting two surface patches in its analysis. On the other hand, purification protocols can be used to improve the quality of the generated entanglements. However, the purification process can itself increase the error rate in the patches by delaying the gate execution. So the right amount of distillation should be performed if necessary. In addition, it is not clear which protocol for entanglement generation and what topology for connecting multiple modules should be used to minimize entanglement generation overhead. We will explore the effect of inter-module entanglement fidelity, local gate time, number of purification rounds, and entanglement generation time on logical error rate. Through simulation and Monte Carlo analysis, we will show what should be the coherence time of qubits on patches of surface code for fault-tolerant distributed quantum computing. 


\myparab{Noise model:}
We assume data qubits in each separate surface patch undergo a time-dependent single-qubit depolarizing channel as in
    \begin{align}
    \label{eq:dec-err-data}
        {\cal E}_t(\rho) = e^{-t/\tau} \rho + \frac{1}{3}(1-e^{-t/\tau_\text{coh}}) \sum_{\sigma=X,Y,Z}
        \sigma \rho \sigma
    \end{align}
We assume ancilla qubits and data qubits at the boundary of a surface code experience noise error $p_b$. In addition, we assume the ancilla qubit measurement error is $p_m$.





%As shown in \cite{ayanzadeh2023frozenqubits} we observe that the majority of qubits in the corresponding algorithm of real-world applications follow the “power-law“ distribution, where some hotspot qubits have a significantly higher number of connections with other qubits. Based on this observation, we do our resource allocation for purification. 


%We can use storage servers to generate and store the entanglements when the resources are idle. Later, the EPR pairs can be used from the storage servers to serve the circuit. In this project, we do not explore the problem of optimally distributing a given quantum circuit for evaluation over a network of QCs. Partitioning the qubits to different processors in a heterogeneous quantum network with the goal of minimizing the overall communication overhead \cite{g2021efficient}. 

%Given a topology of quantum nodes in a quantum data center, how should resources at switches be scheduled to minimize the run time of a circuit? What would be the overhead of orchestrating the resources in a quantum data center?


% \begin{figure}
% \centering
%     \includegraphics[width=8cm]
%     {img/QDC_topology}
%     % \vspace{-0.2in}
%   \caption{Topology of a QDC empowered with quantum storage servers
%   }\label{fig:QDC_topology}
% \end{figure}



    
%The objective is to minimize the number of times that we can not handle the demands of a time slot. Because the more time slots that we can not handle the demands, we have to wait one-time slot to satisfy the entanglement of that moment and the more delay in executing the circuit. In other words, we want to maximize parallelization. We set the objective function as maximizing $-\sum_{t\in T}u_t-d_t$. If we assume the maximum required entanglement between different pairs of nodes is less than he capacity of the storage servers, then we do not need to use this objective function. 








%A surface code is a special type of "stabilizer code" \cite{bravyi1998quantum,dennis2002topological} which due to its relatively high fault-tolerant thresholds is a clear and suitable option for extensive designs in experimentally feasible systems \cite{fowler2012surface,fowler2010surface}. When the connection is established through distributed entanglement between two modules, that entanglement becomes a tool for making non-local, teleported gates between qubits in different modules. \cite{guinn2023co} proposes QuIRC, a superconducting Quantum Interface Routing Card for Lattice Surgery between surface code modules inside of a single dilution refrigerator. QuIRC improves scaling by allowing the connection of many modules, increases ancilla connectivity of surface code lattices, and offers improved transpilation of Pauli-based surface code circuits. Through simulation, the authors analyze collisions in gate schedules and EPR pair generation schedules. On the other hand, \cite{ramette2023fault} performs an analytical analysis and demonstrates that different surface code sections can be linked securely, even when there is considerable noise along the connecting interface. Theoretically and through simulations, the authors analyze and calculate how errors across the interface and within the surface code module collectively impact the system. 




==> qdc.tex <==
\section{A Quantum Data Center}
This section describes different scheduelrs for entangelmt geenration in a quantum data center (QDC), where multiple Quantum Processing Units (QPUs) are interconnected via a high-speed optical quantum network. Our focus is on modeling and evaluating key architectural components such as physical-layer entanglement generation, quantum data center network topology, and resource-aware scheduling under realistic constraints that influence the performance of distributed quantum execution. While other important aspects like quantum memory management, quantum error correction, and classical control signaling are crucial, they fall outside the scope of this work and are left for future exploration.


Figure \ref{fig:components} outlines the end-to-end workflow of our system. Initially, the quantum circuit is partitioned using our optimized algorithm. Then, a network orchestrator schedules entanglement generation for remote gate execution, considering both the circuit dependency graph and network resource constraints. The network connecting QPUs is a switch-centered or server-centric network \cite{shapourian2025quantum} where we have photonic switches and racks to hold QPUs. For intra-rack and cross-rack entangemtn generation we can use different protocols for entangelmt genration that we explain in detail in the next subsection.


\begin{figure}
\centering
    \includegraphics[width=9cm]{img/Clos_cross_rack_intra_rack_pair_gen.pdf}
    \vspace{-0.06in}
\captionsetup{justification=centering} 
  \caption{A Clos topology for a quantum data center and physical model of cross rack and intra rackEPR pair pair geneneration}\label{fig:partitioning_algs}
\end{figure}



\begin{figure}
\centering
    \includegraphics[width=9cm]{img/Opt_WBCP.pdf}
    \vspace{-0.06in}
\captionsetup{justification=centering} 
  \caption{Window-based circuit partitions with intra-window gate packign and state teleportation}\label{fig:partitioning_algs}
\end{figure}





% Common photonic encodings include:

% Fock-state encoding (presence/absence):
% \subsection*{Photonic Qubit Encodings}

% \begin{itemize}
%     \item \textbf{Fock-space encoding (Presence/Absence):}
%     \begin{equation}
%         |1\rangle_p := a^\dagger | \text{vac} \rangle, \quad |0\rangle_p := | \text{vac} \rangle
%     \end{equation}

%     \item \textbf{Polarization encoding:}
%     \begin{equation}
%         |1\rangle_p := a^\dagger_v | \text{vac} \rangle, \quad |0\rangle_p := a^\dagger_h | \text{vac} \rangle
%     \end{equation}

%     \item \textbf{Time-bin encoding:}
%     \begin{equation}
%         |1\rangle_p := a^\dagger_e | \text{vac} \rangle, \quad |0\rangle_p := a^\dagger_l | \text{vac} \rangle
%     \end{equation}
% \end{itemize}




\subsection{Intra and cross rack entanglemt geenration protocols}

The physical layer of the QDC is responsible for generating entangled Bell pairs (EPR pairs) between communication qubits residing on different QPUs. These EPR pairs are the fundamental resource for executing non-local quantum gates and enabling qubit teleportation.

Each QPU contains a set of data qubits (for computation) and communication qubits (for networking). Entanglement is established using photonic interfaces—either through direct photon emission (emitter-emitter schemes) or photon scattering (scatterer-scatterer schemes). These methods produce single-photon states in encodings such as polarization, time-bin, or Fock-space \cite{ang2024arquin,monroe2014large,jiang2007distributed,bayerbach2023bell}.

For cross-rack entanglement generation, we assume a dual-source model: each source emits entangled photons, with one photon sent to a Bell State Measurement (BSM) module and the other routed to a QPU. Entanglement is heralded by three detection events—two for photon arrivals and one successful BSM. Using non-degenerate photon sources (e.g., emitting photons at near-infrared and telecom wavelengths) enables compatibility with QPU hardware and existing fiber infrastructure, avoiding inefficient quantum frequency conversion.


\subsection{Entanglement Generation Scheduling}
\label{sec:schedulers}

\myparab{Scheduling Strategies}
We investigate scheduling strategies for entanglement generation and gate execution in distributed quantum computing, where non-local gates require EPR pairs and gate dependencies are modeled as a directed acyclic graph (DAG). Entanglement generation is probabilistic, and its variability plays a key role in scheduling decisions.

Static Scheduling with Expectation Values (Reference Model):
This model, commonly used in prior work, assumes entanglement generation completes in deterministic time based on the expected value of the success probability. All gates in a layer are executed only after all required EPR pairs are assumed to be available. While analytically convenient, this model smooths over randomness and can underestimate execution latency. We do not implement this model but refer to it as a baseline to contrast with our probabilistic evaluations.
Static Scheduling with Probabilistic Simulation:
In this model, we explicitly simulate the stochastic nature of entanglement generation, where each attempt can succeed or fail according to the given probability. The scheduler follows a strict layer-by-layer execution pattern, advancing only once all gates in the current layer have been supplied with entanglement. This captures the performance degradation due to failed attempts, retries, and resource contention.
Dynamic Scheduling with Probabilistic Simulation:
Our proposed approach embraces the flexibility of dynamic scheduling, where gates are executed as soon as their logical and entanglement dependencies are satisfied—regardless of their original layer. This model allows the system to opportunistically progress through the DAG, making better use of available entanglement resources and reducing idle time caused by network delays or entanglement failures.
\myparab{Why Expectation-based Models Fall Short}
While static scheduling with expectation values can provide a rough estimate of long-term average behavior, it fails to capture critical real-world dynamics such as entanglement failures, queue buildup, and coherence loss due to delays. Especially under constrained or variable conditions, expectation-based models can significantly overestimate system performance. Our work focuses on realistic, probabilistic models to evaluate how scheduling strategies behave under these non-ideal conditions.
Once a circuit is partitioned, a resource scheduler is required to manage entanglement generation over time. This scheduler respects gate dependencies in the circuit DAG and handles resource contention due to limited communication qubits and shared BSM modules. Efficient scheduling ensures EPR pairs are generated and used in a timely manner for remote gate execution or teleportation.

We simulate two scheduling strategies for gate execution following circuit partitioning:

Static Scheduling: All gates in the current DAG front layer (i.e., with no unmet dependencies) are scheduled for execution simultaneously. The DAG is updated only after all gates in the layer complete. This method simplifies control but can lead to idle time if some gates stall due to resource unavailability or longer entanglement generation times.

Dynamic Scheduling: Gates are scheduled as soon as their dependencies are resolved. The DAG is updated incrementally, enabling asynchronous execution. This approach maximizes concurrency and improves resource utilization—particularly in probabilistic networks—but introduces greater complexity in execution state management.

\myparab{Network Orchestrator with Lookahead Capability:}
The network orchestrator can be enhanced in several ways, one of which is by incorporating a lookahead mechanism. In this approach, at each layer of the circuit DAG, the orchestrator examines the nodes in the subsequent $k$ layers and proactively initiates entanglement generation for upcoming non-local gates. If entanglement is successfully established, the communication qubits temporarily store the EPR pairs until those future gates are ready to execute.

However, this strategy comes with trade-offs. Communication qubits typically have limited coherence times, and holding EPR pairs for too long can lead to decoherence, degrading the quality of the entangled states. Our analysis reveals that when coherence times are low, the lookahead strategy provides little to no benefit—and may even increase execution delay by occupying network resources unnecessarily and blocking on-demand entanglement generation.

In Section \ref{sec:eval}, we conduct a detailed numerical evaluation of these scheduling strategies within a realistic quantum data center setup using our custom lightweight event-driven simulator.

% Circuits are modeled as DAGs, where nodes represent quantum gates. Our simulator tracks gate execution timelines, resource contention, and network state across multiple QPUs and racks. The results offer insights into how different scheduling strategies impact overall circuit latency and system throughput under realistic constraints.

==> rel_wk.tex <==
\section{Related work}
We overview the related work on circuit compilation techniques here.


\subsection{Qubit assigning to QPUs}


% Different circuit compilation schemes have been proposed in the literature. 


In quantum circuit compilation, the goal is to split a quantum circuit $C$, consisting of list of operations on a set of logical qubits $q = {q_0, q_1...}$, among a set of QPUs $Q = {Q_0, Q_1...}$ and the goal usually is to minimize inter-QPU entanglement generation that is required to execute two-qubit non-local gates. Converted the circuit to an interaction graph where each qubit corresponds to a node on the graph, while interactions of all pairs of qubits are summed into weighted edges, this can be reduced to  min-cut graph partitioning problem which is NP-hard. 

In recent years, multiple heuristics have been developed for circuit compilation in distributed quantum computing, often relying on methods such as state teleportation, gate teleportation \cite{andres2019automated,houshmand2020evolutionary}, and packing multiple two-qubit gates \cite{wu2022autocomm,wu2023entanglement} to reduce entanglement costs. Gate-teleportation based approaches typically fix qubit assignments at the start of the circuit, limiting flexibility, and require two-way teleportation protocols, where qubits must return to their original QPU after operations. Considering state teleportation on the other hand allows
for changes in qubit allocation during the execution of
the circuit. Recently some approaches have been proposed that merge state and gate teleportation \cite{burt2024generalised,nikahd2021automated}. However, most of these approaches report inter- or only report gate teleportation or state teleportation as the final cost while neglecting the probability nature of entanglement generation and the possibility of parallelization in entanglement generation or have been demonstrated for small number of QPUs \cite{promponas2024compiler,pastor2024circuit}.


Some compilers \cite{tang2021cutqc,peng2020simulating,tang2024distributed,tang2023tensorqc,tang2022scaleqc} have also been proposed to implement DQC
without inter-QPU communications by cutting large circuits into smaller ones and running them on different devices, yet they require
non-scalable classical post-processing




==> removed_content.tex <==



\subsection{Circuit Partitioning}
We build our circuit partitioning algorithm upon two existing strategies: the Window-Based Circuit Partitioning (WBCP) method proposed in \cite{kaur2025optimized} and the time-sliced approach from \cite{baker2020time}. Time-sliced methods can sometimes fail to produce valid qubit assignments within a layer—for example, if a layer with 10 qubits contains five two-qubit gates with no non-overlapping mapping. One workaround is to push certain gates to adjacent layers, which is naturally handled in WBCP where windows can span less than or more than a full layer.

We extend these concepts by introducing additional optimizations—namely, gate packing and intra-partition state teleportation—forming our Optimized WBCP strategy. These enhancements improve parallelism and reduce entanglement overhead across QPUs. The key innovations include:

\textbf{Boundary-Aware Partition Refinement:} To minimize cross-partition communication, we refine the assignment of gates near window boundaries. This reduces the number of non-local two-qubit gates that require remote entanglement. At each window, we check the gates in the first layer of the next window and check if the gate can be executed locally using current window assigning. If so, we include that gate in the gate set of the current window. 

\textbf{Gate Packing Optimization:} This module clusters two-qubit gates that operate on overlapping or adjacent qubits within the same window. We use the embedding conditions proposed in \cite{andres2024distributing} to cehck if two gates can be packed together inside a window. 

\textbf{Intra-Partition State Teleportation:} To handle gate dependencies more flexibly, we allow state teleportation within partitions. This technique is efficient when there are more than two non-local gats between the qubits of two partitions. Figure \ref{fig:partitioning_algs} illustrates the concept of gate packing and teleportation.

\subsection{Circuit partition}
To assess the performance of various circuit partitioning strategies for distributed quantum computing, we conduct simulations on Qiskit-generated benchmark circuits, varying the number of partitions. Each circuit is partitioned using a fixed set of strategies: Kernighan-Lin (KL), the baseline Window-Based Circuit Partitioning (WBCP), our optimized variant (Opt-WBCP), and FGP-roee—an approach introduced in \cite{baker2020time} as a state-of-the-art method. FGP-roee methos maps qubits to QPUs per time slice (i.e., each circuit layer), considering the cost of moving data across layers using a tunable lookahead scheme. It shares similarities with WBCP in its windowed nature, though our method permits windows to include gates from multiple layers. A noted drawback of FGP-roee is its high computational overhead for circuits with many layers.




% \subsection{Circuit Partitioning}
% We build our circuit partitioning algorithm upon two existing strategies: the Window-Based Circuit Partitioning (WBCP) method proposed in \cite{kaur2025optimized} and the time-sliced approach from \cite{baker2020time}. Time-sliced methods can sometimes fail to produce valid qubit assignments within a layer—for example, if a layer with 10 qubits contains five two-qubit gates with no non-overlapping mapping. One workaround is to push certain gates to adjacent layers, which is naturally handled in WBCP where windows can span less than or more than a full layer.

% We extend these concepts by introducing additional optimizations—namely, gate packing and intra-partition state teleportation—forming our Optimized WBCP strategy. These enhancements improve parallelism and reduce entanglement overhead across QPUs. The key innovations include:

% \textbf{Boundary-Aware Partition Refinement:} To minimize cross-partition communication, we refine the assignment of gates near window boundaries. This reduces the number of non-local two-qubit gates that require remote entanglement. At each window, we check the gates in the first layer of the next window and check if the gate can be executed locally using current window assigning. If so, we include that gate in the gate set of the current window. 

% \textbf{Gate Packing Optimization:} This module clusters two-qubit gates that operate on overlapping or adjacent qubits within the same window. We use the embedding conditions proposed in \cite{andres2024distributing} to cehck if two gates can be packed together inside a window. 

% \textbf{Intra-Partition State Teleportation:} To handle gate dependencies more flexibly, we allow state teleportation within partitions. This technique is efficient when there are more than two non-local gats between the qubits of two partitions. Figure \ref{fig:partitioning_algs} illustrates the concept of gate packing and teleportation.



% \begin{figure}
% \centering
%     \includegraphics[width=9cm]{img/Opt_WBCP.pdf}
%     \vspace{-0.06in}
% \captionsetup{justification=centering} 
%   \caption{Window-based circuit partitions with intra-window gate packign and state teleportation}\label{fig:partitioning_algs}
% \end{figure}





% Common photonic encodings include:

% Fock-state encoding (presence/absence):
% \subsection*{Photonic Qubit Encodings}

% \begin{itemize}
%     \item \textbf{Fock-space encoding (Presence/Absence):}
%     \begin{equation}
%         |1\rangle_p := a^\dagger | \text{vac} \rangle, \quad |0\rangle_p := | \text{vac} \rangle
%     \end{equation}

%     \item \textbf{Polarization encoding:}
%     \begin{equation}
%         |1\rangle_p := a^\dagger_v | \text{vac} \rangle, \quad |0\rangle_p := a^\dagger_h | \text{vac} \rangle
%     \end{equation}

%     \item \textbf{Time-bin encoding:}
%     \begin{equation}
%         |1\rangle_p := a^\dagger_e | \text{vac} \rangle, \quad |0\rangle_p := a^\dagger_l | \text{vac} \rangle
%     \end{equation}
% \end{itemize}




==> sim.tex <==
\section{Simulation}
We have the qubits as the leaves of tree connected to QPUS. QUPs are connected to racks. We route from qubits to qubits. The leaves are string while anything else is integer.  If the shortest path between qubits is less than 3, then they are on the same QPU. The number of qubits per node means the number of nodes under the one to the last nod ein the tree and that means the number of qubots per QPU. TO handle different partitioning algorithms, we need to update the topology of the networkj per layer or per dag gate or per successfull attempt such that the leaves (qubits) will be exchanged in the network over time.


==> t_eval.tex <==
\section{Evaluation}

In this section, we evaluate the effectiveness of our proposed optimization modules applied to the WBCP algorithm. The resulting circuit partitions are used as input to our network orchestration framework, where we schedule entanglement generation between different QPUs in a Clos topology to enable remote gate execution and qubit teleportation.


\subsection{Circuit partition}
To assess the performance of various circuit partitioning strategies for distributed quantum computing, we conduct simulations on Qiskit-generated benchmark circuits, varying the number of partitions. Each circuit is partitioned using a fixed set of strategies: Kernighan-Lin (KL), the baseline Window-Based Circuit Partitioning (WBCP), our optimized variant (Opt-WBCP), and FGP-roee—an approach introduced in \cite{baker2020time} as a state-of-the-art method. FGP-roee methos maps qubits to QPUs per time slice (i.e., each circuit layer), considering the cost of moving data across layers using a tunable lookahead scheme. It shares similarities with WBCP in its windowed nature, though our method permits windows to include gates from multiple layers. A noted drawback of FGP-roee is its high computational overhead for circuits with many layers.


We evaluate our approach using a diverse set of circuits, including Quantum Fourier Transform (QFT), Quantum Volume (QV), QAOA, and Random circuits—each with 100 qubits to represent large-scale quantum workloads. These circuits are decomposed into a native gate set (cx, h, rz, crz) using Qiskit's transpile() function to ensure compatibility with realistic hardware constraints.


\begin{table}[ht]
\centering
\caption{Comparison of partitioning costs across different circuit types and algorithms}
\begin{tabular}{|p{1.4cm}|p{0.6cm}|c|c|c|c|}
\hline
\textbf{Circuit} & \textbf{\#QPUs} & \textbf{KL} & \textbf{WBCP} & \textbf{Opt\_WBCP} & \textbf{FGP\_roee} \\
\hline
adder\_n118 & 2 & \textbf{15.0} & \textbf{15.0} & 19.0 & 76.0 \\
bv\_n140 & 2 & 3.0 & 3.0 & \textbf{2.0} & {4.0} \\
bv\_n280 & 2 & 13.0 & 13.0 & \textbf{2.0} & {4.0} \\
cat\_n130 & 2 & 1.0 & 3.0 & \textbf{1.0} & {4.0} \\
cat\_n260 & 2 & \textbf{1.0} & \textbf{1.0} & 3.0 & {4.0} \\
dnn\_n16 & 2 & 16.0 & 16.0 & \textbf{6.0} & {10.0} \\
ising\_n420 & 2 & 6.0 & \textbf{2.0} & 6.0 & \textbf{2.0} \\
square\_root\_n18 & 2 & 130.0 & 130.0 & \textbf{12.0} & 150.0 \\
wstate\_n118 & 2 & \textbf{2.0} & \textbf{2.0} & \textbf{2.0} & 118.0 \\
wstate\_n36 & 2 & 6.0 & \textbf{2.0} & \textbf{2.0} & 36.0 \\
\hline
\end{tabular}
\label{tab:partition_cost_comparison}
\end{table}


The bar plots in Figure \ref{fig:partitioning_algs} compare the average cost across algorithms for fixed circuit types and partition counts. 
%Line plots in Figure \ref{fig:partitioning_algs_window_length} show how the cost evolves as a function of window length.

Figure \ref{fig:partitioning_algs_as_num_qubits} plots the entanglement cost as a function of the number of partitions and qubits. Our method outperforms FGP-roee in structured circuits by effectively packing gates. However, for circuits with high randomness, FGP-roee may yield better results. Notably, FGP-roee fails to partition certain circuits like QV and square-root circuits with 50+ qubits, often entering infinite loops while searching for valid qubit assignments.


% \begin{figure*}
% \centering
%     \includegraphics[width=18.3cm]{img/partitioning_algs_window_length.pdf}
%     \vspace{-0.06in}
% \captionsetup{justification=centering} 
%   \caption{Different circuit partitioning algorithms as window length}\label{fig:partitioning_algs_window_length}
% \end{figure*}



\begin{figure*}
\centering
    \includegraphics[width=18.3cm]{img/bar_plot_KL_WBCP_OptWBCP.pdf}
    \vspace{-0.06in}
\captionsetup{justification=centering} 
  \caption{Different circuit partitioning algorithms}\label{fig:partitioning_algs}
\end{figure*}






\begin{figure*}
\centering
    \includegraphics[width=18.3cm]{img/cost_as_num_qubits.pdf}
    \vspace{-0.06in}
\captionsetup{justification=centering} 
  \caption{Different circuit partitioning algorithms cost as the number of qubits}\label{fig:partitioning_algs_as_num_qubits}
\end{figure*}





\subsection{Network orchestrator}
We now evaluate how realistic assumptions about entanglement generation, topology, and hardware constraints—such as network reconfiguration delay and probabilistic entanglement—affect circuit execution performance in a quantum data center (QDC).

The primary metric is the total time required to generate EPR pairs for remote gates after partitioning, with total latency measured from start to completion of all gates. We focus on KL and Opt-WBCP, using two different entanglement scheduling strategies.

We incorporate realistic hardware assumptions: emitter-emitter protocol with Fock space encoding for intra-rack communication, and scatterer-scatterer protocol for inter-rack links \cite{shapourian2025quantum}. 

Communication qubit count per QPU is 2 by default. Intra-rack entanglement generation success probability is 0.5; cross-rack probability is variable, defaulting to 0.3 unless otherwise stated. Table \ref{table:table2} summarizes all parameters.
We adopt a Clos topology with 4 racks, 2 aggregation switches, and 8 QPUs (see Figure \ref{fig:clos_simulation}). Intra-rack entanglement attempt time is 1 microseconds, while cross-rack attempt time is $10$ ms. Optical switch reconfiguration delay is assumed to be 1 ms.


We explore two gate execution strategies:

\textbf{Static Scheduling:} All executable gates in the current circuit DAG layer are executed simultaneously. The DAG is updated only after the full layer completes. This approach may underutilize resources when some of the EPR pair are generated quickly and need to wait until others are generated.

\textbf{Dynamic Scheduling:} Gates are executed asynchronously as soon as their dependencies are satisfied. This allows increased parallelism and reduced latency, especially under probabilistic gate durations.



For each gate, the system checks the availability of an entangled path (via shortest path routing). If resources are unavailable, execution of that gate is deferred. 




\subsubsection{Delay as network schedulers}

Figure \ref{fig:delay_as_p} shows average circuit delay as a function of cross-rack entanglement success probability ($p$), comparing static (SS) and dynamic (DD) schedulers. The dynamic scheduler reduces delay by improving resource utilization and allowing independent gate progress.




\begin{figure*}
\centering
    \includegraphics[width=18.7cm]{img/delay_as_p.pdf}
    \vspace{-0.06in}
\captionsetup{justification=centering} 
  \caption{Different schedulers for different circuits. SS is for static scheduler and DD is for dynamic scheduler for 8 QPUs each with 2 communication qubits. $p$ is cross rack entanglement generation success probability. Intra-rack ent. gene. p is $\frac{1}{2}$.}\label{fig:delay_as_p}
\end{figure*}

 

\subsubsection{Delay vs resources:}
Figure \ref{fig:dealy_as_bw} shows delay as a function of network resources, specifically the number of communication qubits per QPU and BSMs per switch. Increasing either reduces delay, but only up to a point: if QPUs lack communication qubits, additional switch resources are underutilized, and vice versa.



\begin{figure*}
\centering
    \includegraphics[width=17.3cm]%{img/delay_as_bw.pdf}
    {img/heat_map_resources.pdf}
    \vspace{-0.06in}
\captionsetup{justification=centering} 
  \caption{Circuit execution delay as a function of resources for 8 QPUs and 100 qubits in ach circuit}\label{fig:dealy_as_bw}
\end{figure*}



\subsection{Demand Matrix between QPUs}

Finally, Figure \ref{fig:heat_map_demand} presents a heatmap showing the percentage of entanglement requests between QPUs per circuit. This demand distribution is circuit-dependent and can inform future scheduler designs, much like traffic-aware scheduling in classical data centers \cite{zerwas2024d3}. Most entanglement is between a limited subset of QPUs, influenced by our locality-preserving partitioning.



% \begin{figure}
% \centering
%     \includegraphics[width=9.3cm]{img/cost_delay_ratio_demands_over_t.pdf}
%     \vspace{-0.06in}
% \captionsetup{justification=left} 
%   \caption{The ratio of cost and delay in KL to the cost and delay in Opt\_{WBCP} for QFT and QAOA circuits with 100 qubits and 4 QPUs and 2 BSM on racks and 2 comm qubits.}\label{fig:cost_delay_ratios}
% \end{figure}




\begin{figure*}
\centering
    \includegraphics[width=18.3cm]{img/heat_map.pdf}
    \vspace{-0.06in}
\captionsetup{justification=centering} 
  \caption{Heatmap on QPU-to-QPU entanglement generation for different circuits. Different circuits generate different heatmaps.}\label{fig:heat_map_demand}
\end{figure*}






% \begin{figure}
% \centering
%     \includegraphics[width=8.3cm]{img/coh_t.pdf}
%     \vspace{-0.06in}
% \captionsetup{justification=centering} 
%   \caption{(Cartoon graph)Delay as coherence time (sec)}\label{fig:coh_t}
% \end{figure}



